PeriphAR: Fast and Accurate Real-World Object Selection with Peripheral Augmented Reality Displays

Gaze-based selection in XR requires visual confirmation due to eye-tracking limitations and target ambiguity in 3D contexts. Current designs for wide-FOV displays use world-locked, central overlays, which are not conducive to always-on AR glasses. This paper introduces PeriphAR (per-ree-far), a visualization technique that leverages peripheral vision for feedback during gaze-based selection on a monocular AR display. In a first user study, we isolated text, color, and shape properties of target objects to compare peripheral selection cues. Peripheral vision was more sensitive to color than shape, but this sensitivity rapidly declined at lower contrast. To preserve preattentive processing of color, we developed two strategies to enhance color in users' peripheral vision. In a second user study, our strategy that maximized contrast of the target to the neighboring object with the most similar color was subjectively preferred. As proof of concept, we implemented PeriphAR in an end-to-end system to test performance with real-world object detection.

==> backup/study1.tex <==
\section{Study 1 Reflection \& Takeaways}

Here, we contextualize the results with participant feedback, sharing our observations and a design rationale for our second study.

% Color
\p{Color the most potent feature}
Overall, the tetris game showed a strong trend in favor of the color condition, performing the best in terms of both task performance and subjective ratings, as well as overall preference.
Several participants argued the advantages of the color condition, \eg
P10: ``I liked the fact that the color showed up in the center of the display, it made it a lot easier. It seemed I was using the mini display more peripherally, not looking directly at it. It seemed that seeing it peripherally communicated quicker to my brain.''
P27: ``It was just a manageable amount of information for my peripheral [..]. It was easier to interpret.''
P13: ``It's my preference, maybe because of my age [45 years] but it's bright and it attracts my attention.''

The main goal of our first study was to understand how each feature---text, color, shape, and animation---contributes to task and subjective performance, relative to the snapshot condition as a baseline. Given that color was so dominant in our tetris game, we considered developing a peripheral display for real-world objects based on algorithms for color extraction from passthrough images for our second study. However, we quickly realized that designing and studying such algorithms would need significant, new research (\cf Section~\ref{sec:discussion}). Additional reasons not to make color our focus was limited control of our display emulation over optical parameters (\eg light refraction), as well as the relatively high error rates.

% Other features
\p{Color by itself not sufficient} During the tetris game, most participants encountered at least one block with nearby tetrominoes of similar color, sometimes even with overlapping shapes. This often prompted participants to reflect on the limitations of a color only peripheral display. We observed two trends: switching preferences or suggesting combining features.
P32 who preferred shape: ``There wasn't the shapes at the side panel, a little jumbled on the left side, trying to discern between the ones that were closely together, was a little difficult to pick.''
P37 who preferred snapshot: ``This was all circles, no writing, just showed the colors that I was looking at, the one with the writing was more helpful.''
P38 who preferred text: ``Having just the letter on there was less busy because I just see that out of my periphery for the most part so it was less distracting, maybe, and you can just do the visual cues on it, but I do reference that when your eyes are in the right spot that letter matches it, so with that big cluster on the left shelf that helped me there a lot.''
P34 who preferred text: ``the letter one [text] is still my preference but there were times where the colored one seemed better when there are shapes with colors that are not close in the color spectrum, but I think the most consistently helpful configuration was the letter for me.''
P38 suggested combining text and shape: ``I guess the biggest difference was the grayed out shape box in the display, I still like the letter but that would probably be my next choice, I think because it is less obtrusive, like the letter and the grayed out shape are less distracting and obtrusive than having the color competing in your peripheral field.''
P29 who preferred text suggested combining it with color: ``it was real easy to see, I liked the letter, the only thing I would change is that I would make them colored, it was just that your eyes don't have to go as far because it was just in the top left corner as opposed to the middle of the mini display.''
P11: who overall preferred color also said ``I'd prefer to see shape and color.''

% Snapshot
\p{More context not always better} The snapshot condition was preferred by some participants ``because with just the color it was a little hard when the same objects with the same color were close together. I liked that I had all of the things, so it was easier to tell what you're looking at'' (P20), and ``because it showed the shape and color that was like I thought more helpful than just the color'' (P19).
P35: ``I feel like with the [snapshot] because the mini display there is more going on, the other way I could just pay attention to the colors in the peripheral, whereas with this one I noticed myself I needed to jump to the display to verify more, I like it more even though I have to look at it more than with just the color.''
However, the majority of participants felt that it contained too much, \eg
``it was really distracting, felt more in the way than any of the previous, felt a lot slower with this one, was a lot more difficult to select the targets,'' (P7), ``was a little complicated, there was a lot of stuff in the box so I didn't do that well'' (P15), and it ``had more of the shapes and the colors that were surrounding the letter I was looking at, didn't like it because it distracted me from finding what I was looking at'' (P10).
Some participants appreciated that it contained multiple features but still suggested changes, \eg  P7: ``too much in the box, felt like it was zoomed in and that was confusing, would overall still prefer shape and color. I don't like the letter but some people may do, would prefer for the letter to be bottom right''.
P21: ``The biggest difference is that there is a thumbnail---more information that you need that is not significant---one good thing about it is that you can see the shape of the thingy you are looking at instead of only color'' (P21).
P16: ``It showed actual shape which I liked but I didn't like that it showed its position in 3D by showing other things around it, because when you're seeing it from the peripheral with the other colors and shapes around it was confusing. I also liked that it showed the letter. While I liked that it showed the shape I still found seeing the color alone easier.''
Because color was such a potent feature, seeing multiple colors in the peripheral vision was ``confusing,'' P24 said, ``a lot of color in there, and sometimes I'm not really sure which one they mean, sometimes in the left and I try to peak at the back it doesn't work it says I'm looking at something in the front instead.''
Also seeing multiple shapes was confusing, as explained by
P31: ``I noticed that if there were multiple objects near it they were all showing up, that was very confusing, I guess they were trying to provide some context or visual anchor, but I couldn't tell what object I was looking at, probably too much information in that. I stopped looking at the mini display after a while because the information was confusing, it made me click the button too fast because I could see it in the display but it wasn't actually on it, I guess I should have used the letter but I just wasn't, but definitely seeing multiple shapes that got confusing for me.''
P32: ``The side display was really cluttered, there was too many objects on there so it was hard to tell if the actual one that I was looking at was shown in the display.''

% Animation
\p{Sensitive to dynamic features but hard to tell the difference}
As a way to address the issue of the display being overloaded, we developed dynamic features in the form of different animations.
Based on the memory game and tetris (Part 2), we had two main observations. First, in line with prior work \cite{Luyten-CHI16}, participants were sensitive to animation in the peripheral display. Second, and unique to our work, syncing dynamic features with gaze behavior is a major new challenge.
We say this because, when returning to tetris after the memory game intervention, participants clearly noticed the differences in display behavior. However, only a few participants detected the differences between both the memory conditions and between the tetris (Part 2) conditions.

% Memory
P19 said ``it felt easier'' with the transition condition but didn't notice the specific differences to fixation.
P20 who didn't notice a difference initially when trying transition after fixation, but then ``it seemed like the monster popped up faster when I looked at the ring.'' P38: ``I felt like I had to look at it a little more, don't know if I really have a preference between the two, both kind of equal, I also felt like it was more responsive, like quicker, stuff was popping up a little quicker, it was quicker to populate the monster, but still between the two, I think I'm really swayed between either one, it really depends how you wanna play it.''

% Tetris (Part 2)
Many participants responded positively and more than half (17) even changed their preference to the animation or ambient conditions, \eg
P15: ``I liked how [animation] zoomed through the different shapes in the display.'' P21: ``By far the most comprehensive configuration, the visual, the text, the shape, the peripheral and everything. I feel like it's so much better than [snapshot] because it has the animation and the animation makes the most difference because it imitates the eye tracking movement that I'm doing so I don't have to look at the display to know it's the right one. I'm choosing because my peripheral sight saw that it was moving to the right thing, so I just had to check the color peripherally.''

For the participants that stuck with the static conditions from tetris (Part 1), comments indicated they could not exactly characterize the dynamic feature. Several noted it felt slower, \eg P9: it ``was lagging a bit.''
``I was using both in tandem, objects in world and mini display,'' P31 said, ``sometimes it would look on the object super fast, and other times there was a little bit of a delay, I'm guessing it had to do with having multiple objects together, maybe it had to do a bit more processing to figure out which one I was looking at?''
P7: ``my eye movement and selecting the object was much quicker than the display was feeding the information.''
P22, who did not change, said: ``I noticed that this time it comes zoomed in on the shape and it moves from shape to shape, but I think the color one is still my top choice, because this was slower than how I was looking at things, but it helped me figure out what I was looking at and that my eyes were tracked in the right space.''

On the other hand, P21, who changed their preference in favor of animation, argued: ``I feel like since there is the animation, people would be aware, so people know the system status, there is a little bit of latency but you would know that you are giving it commands, unlike [snapshot] where I felt lost sometimes because I didn't know whether it has detected my eye gaze or not.''
Following this logic and based on the overall performance improvements, we decided to focus our second study on effects of dynamic behavior with real-world objects.

\begin{comment}
\p{Dynamic features with side effects}
For participants that were focused on individual features like text, animation seemed to work against them. P34: ``I think this was like the [snapshot], maybe it just moves the camera towards the object instead of showing the image, I feel like it made it harder to see the letter at the top left.''
Some participants argued that animation introduced additional complexity they thought overall was not necessary, at least not for the tetris game.
P35: ``It's interesting the way the shapes move, I liked the way the mini map/the screen moved in relation to how your eyes moved, allowed you to verify your motion [..]. I feel like even though it was busy, because I was able to reference my previous position, I would say, yeah, it was easy, I like that. I like the spatial reference to the previous selection [..] but I still think I was faster with just the letter [text].''

A few participants felt the animation and adaptive conditions were more 3D, \eg P32: ``[animation] looked it was more 3D, it felt more like it was pointing right at me, as far as the information on the right side panel it was probably the best configuration, the 3D effect and it decluttered a lot, on the left side it was still tough because it was really close.''
P10 said the same about ambient, ``I think the display was more 3D. When I was looking at the condensed shapes, it almost felt like the display was only showing the shape I was looking, but then it still showed the surrounding ones, so it was all there.''
More 3D was not always considered better, \eg P14: ``felt like I was looking at it from a different perspective, so had to match it in my brain.''
Both participants had strong reactions when they tried animation last: 
P14: ``didn't like that, too much going on in the mini display, it was confusing and also distracting.'' P10: ``this last one, I don't know why but things were not registering. I don't know if it was different but I noticed the [text] letter and the shape in the display.''
In the second study, we therefore kept the static features and focused our investigation on the benefits and drawbacks of a gaze adaptive display.
\end{comment}

\p{Gaze adaptive both a challenge and an opportunity}
% pro static
Participants who still preferred the static conditions mostly saw challenges, as it ``felt a little awkward because the display changed a lot,'' P5 said, feeling that ``the transition was less subtle [compared to animation] and more distracting.'' P24 also struggled to get used to the gaze reactive behavior: ``I think there is a layer, whatever you look at is gonna pop up more, [but] I'm not sure I like it more.''
P38 still kept with text because ``[animation] was more busy, I would not say that I prefer this one, I liked the letter and the grayed out shapes, those would be my top choices,'' and for ambient P38 said, ``I didn't notice a lot of difference between this one than the other one, maybe stuff felt a little bit more 3D, there was not a lot stand out for it, between the two I would probably prefer this one, it seemed more 3D, but I can't say that I referenced it either.''

The close rankings of the animation and ambient conditions also showed in many of participants' comments who had a hard time deciding between the two.
% pro animation
P21, who still overall preferred animation, said: ``at first I didn't notice any differences, but then I realized that when you look at the display it'll zoom out so you can see the shape in context. The biggest difference is whether you want to look at the display box. For me, I didn't want to [..] and I think if you want to look at it, it would be a more invasive design.'' They kept with animation as it ``was more efficient because I didn't' have to look at the display box, this one is like [snapshot] plus you can inspect the display box, which is kind of inefficient for me.''
Similarly, P30 argued that ``the way [animation] works is when I looked at the objects, it would also show it in minuscule at the bottom that I moved from that shape to that shape. I noticed that when I looked at another shape it would also follow along with me. That was pretty neat.'' But, for ambient, P30 noticed the peripheral animation was missing and the zoom on world$<>$display transition too subtle/fast: ``when I was looking at the bottom right it showed where I was going [with animation] instead of just popping up on the screen [with adaptive].''
P12 saw the potential with adaptive: ``combined the best of previous conditions, so I prefer this, nicely isolated the shape in the mini display.'' However, P12 then didn't notice the difference to the adaptive when trying animation, but felt a little more accurate, so picked that one as their overall preference.

% pro ambient
P23 was of the opposite opinion, justifying ambient as their top choice:
``I think there is a difference, I felt faster, more efficient. As far as the box, it felt less of a strain to see it and find it, still a little bit of an issue when there's a lot of shapes around, and I need to adjust my head a little bit but I found it was a little better than any of the previous ones. For animation, P23 said, ``not as good as the previous one for some reason, felt a little more clunky, the display to the right just didn't seem as noticeable.''
P27, after switching from text, to snapshot, to color, finally chose ambient as their overall preference: ``I had the snapshots again, the text, the color, the shape, the snapshot of the other shapes around it. I told myself I will not look at this mini display, I will do this entirely by keeping it just in the periphery. This time around I liked it better, [snapshot] had so much information to it.'' P27 seemed to appreciate the ambient mode of the display which initially zoomed in on the target: ``It was easy to see out of my peripheral, the text so I knew I was looking at the right shape, even though I didn't process the shape I saw the color and knew I was looking at the right color.''

Seeing the split among participants but performance improvements with both, we decided to combine the animation and ambient features in the second study and made the difference in whether the display was gaze reactive or not.

==> backup/study2-results.tex <==
\section{Study 2 Reflection \& Takeaways}

The two conditions in the objects task differed in that the ambient condition did not react to gaze shifts towards the display, while the immersive version gradually zoomed in as the user foveated towards the display. While the zoom effect is clearly visible when looking at it straight (\eg in our first-person video recordings), it turns out that this is much harder to tell from the peripheral vision.

\p{Differences hardly noticeable}
Only two participants noticed a difference. P5 said ``it looked like it was zooming in and out, like it was moving in and out in the mini display.'' P9 felt ``it was slower, the response was slower. I preferred the first version [ambient], it was a little bit less jerky.'' The remaining participants all could not tell the difference and some remained neutral about their preference.
P8 who was neutral: ``I choose no because I didn't notice any differences.''
P6: ``this felt pretty similar [..], since it's in my peripheral it's hard to tell the difference, maybe because it's so far off to the right [..] I do feel I was able to make both work pretty well.''
P7 who preferred the immersive version: ``I didn't notice a difference in the display. I noticed a difference in my behavior, felt like I was looking at the display more [in the ambient condition].''

\p{Just ambient less busy}
While there was no winner, one participant that preferred the ambient over the immersive condition did not appreciate the adaptive zoom.
P5 (who noticed the difference): ``if i had to pick I would pick the first one [ambient], it doesn't seem too busy, with the display zooming the object the second one just seemed too busy.''
Others made their choice based on how they felt about their performance, not based on differences since they could not tell, \eg
P11: ``[the ambient condition] felt a little smoother, I felt like I wasn't straining myself as much, not sure if that was just me becoming more used to it or better at it, but it did feel smoother.''

\p{Immersive for tricky cases}
The immersive version helped double check. P7: ``I feel for the unique objects in the room, just seeing the change in color, and that sound it makes is definitely enough, also maybe for the remote, sphere, and tray, there are not many objects nearby, if I look at it [peripherally] and there is a sound and color change I'm confident, but for the flowerpots, I need to check the display and make sure that the object is in the center of the monocular display. When I looked at the monocular display I was most of the time clear which object is being selected, when I looked at the small objects it sometimes contains both of them but it's centering on the one that I'm currently looking at so it was pretty clear what is being selected.''

For the cards task, we included the binocular condition as the baseline, while the monocular display without passthrough was the control and the one with adaptive passthrough experimental. The binocular condition was preferred for various reasons, \eg, P3: ``because I don't have to strain my eye to look at the mini display.'' ``It felt like easier to gaze at an object and see the low/high price because the display isn't in the corner it was right in front of me,'' (P5) ``instead of changing my gaze to the box to see whether the item was high or low, and then losing track of the item'' (P9). P11: ``Everything felt just much simpler, being somebody who is still relatively new to VR it felt a little easier to comprehend and navigate.''
Several participants still argued in favor of monocular with adaptive passthrough and three even preferred it over binocular.

\p{Adaptive passthrough a visual aid}
When asked to describe the MR experience, participants compared adpass to assistive technology, \eg P5: ``it looked like there was a little picture of the object in the display [..] I was picking out real objects with a virtual aid, being the display, with a visual of the object. I preferred it because I liked the visual aid, that helped along with the lower/higher price.''
P7 argued that ``yellow and green are very confusing, in the peripheral view they look the same. [..] I think if all conditions are the same device, I would prefer to render it directly on the object [as in binocular]. But compared to the only price tag [monocular condition], now [with adpass] I was more sure which object I was selecting.'' Without adpass, ``when I was looking at a more cluttered area, even if I knew I selected the low price item, I wasn't entirely sure which item I selected, so I knew I selected something that had the low price but I didn't know which one.''
With adpass, ``I felt less confused about the yellow/green color, probably because I checked the mini display more often anyway, but I feel like in terms of frequency I looked at it more often, but in terms of duration or the amount of attention I paid it was less than [monocular], so more often but easier [with adpass].''

\p{Adaptive passthrough walking a fine line}
Participants that first tried adpass before the monocular condition with it noted its absence. P10: ``What the heck? There is no picture there. I don't like that, I don't like that at all,'' (between the two spheres) ``hopefully it's the right sphere.'' Some who first tried monocular without adpass thought with adpass then was more complex and required effort.
P11: ``that was trickier for me to see in the mini display, I could get used to it as the studies progressed, but it wasn't as smooth as the previous one. I had to really toggle to the mini display intentionally, as a response as I hover an item, I like the click, I appreciate that, but I had to really look over compared to the previous one.''
Three participants favored the adpass condition overall.
P12: ``I liked it better than the first one [monocular] but not than the second one [binocular], the first one was just harder to see the value and continue looking at the object, but I think this one [with adpass], if I'm not mistaken, also showed the object in the box, so that was super helpful.'' 
The main reservations stemmed from the peripheral display being out-of-focus. P12: ``compared to [binocular] it was a little harder because I had to move my eyes to the object, to the box, that was a little more straining, but it wasn't horrible.''
Three participants preferred it over the binocular condition, \eg
P10: ``the first one [with adpass] is best in my opinion, that it shows what it is [through the image] instead of just the text---it almost felt like too easy, I don't know what you really want AR for, like for business purposes maybe you want it that easy, but if you're playing a game, like hell no, I don't want it that easy.''
